Sim-to-Real gap in RL: Use Case with TIAGo and Isaac Sim/Gym

This paper explores policy-learning approaches in the context of sim-to-real transfer for robotic manipulation using a TIAGo mobile manipulator, focusing on two state-of-art simulators, Isaac Gym and Isaac Sim, both developed by Nvidia. Control architectures are discussed, with a particular emphasis on achieving collision-less movement in both simulation and the real environment. Presented results demonstrate successful sim-to-real transfer, showcasing similar movements executed by an RL-trained model in both simulated and real setups.

==> graphs/old/Sim2Real.tex <==
Evolution of the configuration in each joint for a trained agent in Isaac Gym and Isaac Sim compared to its performace on the real TIAGo doted with a low-pass filter $(curre value = curr value*0.998 + new value*0.002)$

For the following picture, time-scales had to be readjusted due to the low-pass filter on the real TIAGo.

\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_1\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=north east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF1_cor] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF1] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_1\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=north east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF1_cor] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF1] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_2\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF2] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF2] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_2\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF2] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF2] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_3\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF3] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF3] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_3\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF3] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF3] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_4\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=north east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF4] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF4] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_4\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=north east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF4] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF4] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_5\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF5] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF5] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_5\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF5] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF5] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}\\
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_7\_joint (Isaac Gym)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t1, y=RDOF7] {\isaacGymData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t2, y=Gym_DOF7] {\isaacGymData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{axis}[
            height=0.2\textheight, % Set the width of the plot
            title={arm\_7\_joint (Isaac Sim)},
            xlabel={Time (s)},
            ylabel={Joint Position (rads)},
            legend pos=south east,
            legend style={nodes={scale=0.5, transform shape}},            
            grid=major,
            title style={font=\footnotesize},
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
        ]
        
        \addplot[black,line width=0.3mm] table[x=t3, y=RDOF7] {\isaacSimData};
        \addlegendentry{real}

        \addplot[gray,line width=0.3mm] table[x=t4, y=Sim_DOF7] {\isaacSimData};
        \addlegendentry{training}

        \end{axis}
    \end{tikzpicture}
    \caption{Responses for TIAGo's arm in the real robot (up), in Isaac Gym (mid) and Isaac Sim (bot) to a step input in each joint of the arm.}
    \label{fig:individual_resp}
\end{figure}

==> graphs/old/bench.tex <==
% \begin{figure}[ht]
%     \centering
%     %\includegraphics[width=0.495\linewidth]{img/IG-response.png}
%     %\includegraphics[width=0.495\linewidth]{img/IS-response.png}
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=0.495\linewidth, % Set the width of the plot
%             title={Multi-joint step (Isaac Gym)},
%             xlabel={Time (s)},
%             ylabel={Joint Position (rads)},
%             legend pos=south west,
%             legend style={nodes={scale=0.5, transform shape}},
%             grid=major,
%             title style={font=\footnotesize},
%             label style={font=\footnotesize},
%             tick label style={font=\footnotesize},
%         ]
        
%         \addplot[orange,line width=0.3mm] table[x=t, y=IG1] {\mydata};
%         \addlegendentry{IG1}

%         \addplot[gray,line width=0.3mm] table[x=t, y=IG2] {\mydata};
%         \addlegendentry{IG2}

%         \addplot[yellow,line width=0.3mm] table[x=t, y=IG3] {\mydata};
%         \addlegendentry{IG3}
        
%         \addplot[blue,line width=0.3mm] table[x=t, y=IG4] {\mydata};
%         \addlegendentry{IG4}

%         \addplot[red,line width=0.3mm] table[x=t, y=IG5] {\mydata};
%         \addlegendentry{IG5}

%         \addplot[green,line width=0.3mm] table[x=t, y=IG6] {\mydata};
%         \addlegendentry{IG6}

%         \addplot[brown,line width=0.3mm] table[x=t, y=IG7] {\mydata};
%         \addlegendentry{IG7}

%         \end{axis}
%     \end{tikzpicture}
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=0.495\linewidth, % Set the width of the plot
%             title={Multi-joint step (Isaac Sim)},
%             xlabel={Time (s)},
%             ylabel={Joint Position (rads)},
%             legend pos=south east,
%             legend style={nodes={scale=0.5, transform shape}},            
%             grid=major,
%             title style={font=\footnotesize},
%             label style={font=\footnotesize},
%             tick label style={font=\footnotesize},
%         ]
        
%         \addplot[orange,line width=0.3mm] table[x=t, y=IS1] {\mydata};
%         \addlegendentry{IG1}

%         \addplot[gray,line width=0.3mm] table[x=t, y=IS2] {\mydata};
%         \addlegendentry{IG2}

%         \addplot[yellow,line width=0.3mm] table[x=t, y=IS3] {\mydata};
%         \addlegendentry{IG3}
        
%         \addplot[blue,line width=0.3mm] table[x=t, y=IS4] {\mydata};
%         \addlegendentry{IG4}

%         \addplot[red,line width=0.3mm] table[x=t, y=IS5] {\mydata};
%         \addlegendentry{IG5}

%         \addplot[green,line width=0.3mm] table[x=t, y=IS6] {\mydata};
%         \addlegendentry{IG6}

%         \addplot[brown,line width=0.3mm] table[x=t, y=IS7] {\mydata};
%         \addlegendentry{IG7}

%         \end{axis}
%     \end{tikzpicture}
%     \caption{Responses for TIAGo's arm in Isaac Gym (left), Isaac Sim (right) to a step input in each joint of the arm.}
%     \label{fig:stepResponse}
% \end{figure}



% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=0.3\linewidth, % Set the width of the plot
%             title={Multi-joint step (Real TIAGo)},
%             xlabel={Time (s)},
%             ylabel={Joint Position (rads)},
%             legend pos=south east,
%             legend style={nodes={scale=0.5, transform shape}},            
%             grid=major,
%             title style={font=\footnotesize},
%             label style={font=\footnotesize},
%             tick label style={font=\footnotesize},
%         ]
        
%         \addplot[orange,line width=0.3mm] table[x=t0, y=DOF1_corr] {\BenchData};
%         \addlegendentry{TA1}

%         \addplot[gray,line width=0.3mm] table[x=t0, y=RDOF2] {\BenchData};
%         \addlegendentry{TA2}

%         \addplot[yellow,line width=0.3mm] table[x=t0, y=RDOF3] {\BenchData};
%         \addlegendentry{TA3}
        
%         \addplot[blue,line width=0.3mm] table[x=t0, y=RDOF4] {\BenchData};
%         \addlegendentry{TA4}

%         \addplot[red,line width=0.3mm] table[x=t0, y=RDOF5] {\BenchData};
%         \addlegendentry{TA5}

%         \addplot[green,line width=0.3mm] table[x=t0, y=RDOF6] {\BenchData};
%         \addlegendentry{TA6}

%         \addplot[brown,line width=0.3mm] table[x=t0, y=RDOF7] {\BenchData};
%         \addlegendentry{TA7}
%         \end{axis}
%     \end{tikzpicture}
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=0.3\linewidth, % Set the width of the plot
%             title={Multi-joint step (Isaac Sim)},
%             xlabel={Time (s)},
%             ylabel={Joint Position (rads)},
%             legend pos=south east,
%             legend style={nodes={scale=0.5, transform shape}},            
%             grid=major,
%             title style={font=\footnotesize},
%             label style={font=\footnotesize},
%             tick label style={font=\footnotesize},
%         ]
        
%         \addplot[orange,line width=0.3mm] table[x=t0, y=SDOF1] {\BenchData};
%         \addlegendentry{IS1}

%         \addplot[gray,line width=0.3mm] table[x=t0, y=SDOF2] {\BenchData};
%         \addlegendentry{IS2}

%         \addplot[yellow,line width=0.3mm] table[x=t0, y=SDOF3] {\BenchData};
%         \addlegendentry{IS3}
        
%         \addplot[blue,line width=0.3mm] table[x=t0, y=SDOF4] {\BenchData};
%         \addlegendentry{IS4}

%         \addplot[red,line width=0.3mm] table[x=t0, y=SDOF5] {\BenchData};
%         \addlegendentry{IS5}

%         \addplot[green,line width=0.3mm] table[x=t0, y=SDOF6] {\BenchData};
%         \addlegendentry{IS6}

%         \addplot[brown,line width=0.3mm] table[x=t0, y=SDOF7] {\BenchData};
%         \addlegendentry{IS7}
%         \end{axis}
%     \end{tikzpicture}
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=0.3\linewidth, % Set the width of the plot
%             title={Multi-joint step (Isaac Gym)},
%             xlabel={Time (s)},
%             ylabel={Joint Position (rads)},
%             legend pos=south east,
%             legend style={nodes={scale=0.5, transform shape}},            
%             grid=major,
%             title style={font=\footnotesize},
%             label style={font=\footnotesize},
%             tick label style={font=\footnotesize},
%         ]
        
%         \addplot[orange,line width=0.3mm] table[x=t0, y=GDOF1] {\BenchData};
%         \addlegendentry{IG1}

%         \addplot[gray,line width=0.3mm] table[x=t0, y=GDOF2] {\BenchData};
%         \addlegendentry{IG2}

%         \addplot[yellow,line width=0.3mm] table[x=t0, y=GDOF3] {\BenchData};
%         \addlegendentry{IG3}
        
%         \addplot[blue,line width=0.3mm] table[x=t0, y=GDOF4] {\BenchData};
%         \addlegendentry{IG4}

%         \addplot[red,line width=0.3mm] table[x=t0, y=GDOF5] {\BenchData};
%         \addlegendentry{IG5}

%         \addplot[green,line width=0.3mm] table[x=t0, y=GDOF6] {\BenchData};
%         \addlegendentry{IG6}

%         \addplot[brown,line width=0.3mm] table[x=t0, y=GDOF7] {\BenchData};
%         \addlegendentry{IG7}
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Responses for TIAGo's arm in the real robot (up), in Isaac Gym (mid) and Isaac Sim (bot) to a step input in each joint of the arm.}
%     \label{fig:stepResponse}
% \end{figure}





